Galaxies and Their Environment at $z \gtrsim 10$ -- I: Primordial Chemical Enrichment, Accretion, Cooling, and Virialization of Gas in Dark Matter Halos

Recent observations made using the James Webb Space Telescope have identified a number of high-redshift galaxies that are unexpectedly luminous. In light of this, it is clear that a more detailed understanding of the high redshift, pre-reionization universe is required for us to obtain the complete story of galaxy formation. This study is the first in a series that seeks to tell the story of galaxy formation at $z \gtrsim 10$ using a suite of large-scale adaptive mesh refinement cosmological simulations. Our machine-learning-accelerated surrogate model for Population III star formation and feedback, StarNet, gives us an unprecedented ability to obtain physically accurate, inhomogeneous chemical initial conditions for a statistically significant number of galaxies. We find that of the 12,423 halos in the mass range of $10^6\,\,M_\odot < M_\mathrm{vir} < 10^9\,\, M_\odot$ that form in our fiducial simulation, $16\%$ are chemically enriched by Population III supernovae by $z\sim12$. We then profile and compare various cooling processes at the centers of halos, and find a complete absence of atomic cooling halos. All of our halos with central cooling gas are dominated by H$_2$ cooling, metal cooling, or a mixture of the two, even in the presence of a strong H$_2$-photodissociating Lyman-Werner background. We also find that gas accretion through the virial radius is not driven by cooling. We find that gas virialization in halos with $M_\mathrm{vir}\gtrsim10^7\,\,M_\odot$ is supported by bulk turbulent flows, and that thermal energy accounts for only a small fraction of the total kinetic energy. Because of this, the mean gas temperature is well below the virial temperature for these halos. We then compute the mass of gas that is available for Population II star formation, and infer star formation rates for each potential star-forming halo.

==> Figures/AccretionCooling/vdisp_blurb.tex <==
\textcolor{olive}{As a measure of turbulence in the halos, we plot average profiles of gas velocity dispersion, with both radial and tangential components, in Figure \ref{fig:vdisp_profiles}. All values are scaled by the virial velocity dispersion, which we calculate as 
\begin{equation}
    \sigma_\mathrm{vir} =  \sigma_\mathrm{1} \sqrt{3},
\end{equation}
where $\sigma_\mathrm{1}$ is the 1-dimensional virial velocity dispersion derived in Section 2.1 of \cite{Bryan_1998} for the case of $\Omega_\mathrm{R}=0$. The halos in the high-mass bin have dispersions roughly equal to the virial value down to $r/R_\mathrm{vir}\approx0.2$, at which point the mean dispersion increases slightly to $\sigma/\sigma_\mathrm{vir}\approx1.25$ (1.5 for metal-cooling halos). The moderate-mass bin shows dispersions that are generally below virial value at all radii, with a wide spread in the central value. The low-mass bin shows a wide spread in velocity dispersion at all radii, which is because the low-mass halos have shallow potential wells, and the gas trapped within the virial radius is thus more susceptible to influences from the environment. The radial component of the velocity dispersion (second row) is below the virial value by roughly a factor of 2 at all radii for the two highest mass bins, suggesting that these halos are marked by smooth radial accretion onto the center. This is somewhat true for the low mass bin as well, though there is still a large spread in the values, with normalized dispersions ranging from 0.25 to 1.5.}
